Open-vocabulary Object Segmentation with Diffusion Models

The goal of this paper is to extract the visual-language correspondence from a pre-trained text-to-image diffusion model, in the form of segmentation map, i.e., simultaneously generating images and segmentation masks for the corresponding visual entities described in the text prompt. We make the following contributions: (i) we pair the existing Stable Diffusion model with a novel grounding module, that can be trained to align the visual and textual embedding space of the diffusion model with only a small number of object categories; (ii) we establish an automatic pipeline for constructing a dataset, that consists of {image, segmentation mask, text prompt} triplets, to train the proposed grounding module; (iii) we evaluate the performance of open-vocabulary grounding on images generated from the text-to-image diffusion model and show that the module can well segment the objects of categories beyond seen ones at training time; (iv) we adopt the augmented diffusion model to build a synthetic semantic segmentation dataset, and show that, training a standard segmentation model on such dataset demonstrates competitive performance on the zero-shot segmentation(ZS3) benchmark, which opens up new opportunities for adopting the powerful diffusion model for discriminative tasks.

==> sec/05-result.tex <==
\hiddensection{Results}
\hiddensubsection{Grounding generation}
% show the main result: our segmentation module output the segmentation results when the stable diffusion output the generated image given the text (prompt). Table: mIOU in  Pascal 16 seen/4 unseen, Coco 65 seen/15 unseen. Figure.
% -----------------------------------
\input{tab/main_ex1.tex}
% -----------------------------------

% \subsection{Reference grounding}
% show the reference grounding results: \em{i.e.}, given the image from the real-world dataset, \em{e.g.}, Pascal, Coco, and the described text (caption/prompt), our segmentation module can output the predicted segmentation results. The results need to be compared with other existing segmentation methods.
% \subsection{Improving other segmentation method with our generated grounding results}
% compare the performance of other segmentation methods before and after adding our generated grounding results to the training dataset.

\hiddensubsection{Comparison with Open-vocabulary methods}

\hiddensubsection{Ablation study}
\paragraph{Training setting}
% -----------------------------------
\input{tab/ablation-1.tex}
% -----------------------------------
\paragraph{Training data}

% -----------------------------------
\input{tab/ablation-2.tex}
% -----------------------------------


% -----------------------------------
\input{tab/main_ex3}
% -----------------------------------
